Model Independent Search For New Physics At The Tevatron

This thesis is a global, model-independent search for new physics, performed with CDF Run II data. The Standard Model prediction is implemented in all final states simultaneously, and an array of statistical probes is employed to search for significant discrepancies between data and prediction. The probes (also known as "Vista", "Sleuth" and "Bump Hunter") are sensitive to population discrepancies, shape disagreements in distributions of kinematic variables, excesses of events of high total transverse momentum, and local excesses of data suggesting resonant production of new massive particles. The result of this search, first in 1 fb-1 and then in 2 fb-1, is null, namely no considerable evidence of new physics was found.

==> pmiss.tex <==
\chapter{Missing Momentum}
\label{sec:pmiss}

Neutrinos, being neutral leptons, traverse the detector leaving no trace, except for the momentum they carry, which appears to be missing from the total momentum of the final state of the event, making it unequal to the initial total momentum.

The reconstruction and measurement of the missing momentum of each event is important, since neutrinos are produced abundantly in weak processes and in many proposed theories beyond the SM there are elusive particles leaving the same signature.

Unlike $e^+e^-$ collider experiments, at CDF the exact initial momentum of the system of interacting hadrons is not precisely known, as each parton carries a varying portion of the longitudinal momentum of the (anti)proton it belongs to, known as Bjorken\index{Bjorken $x$} $x$.
%\footnote{The probability distributions of $x$ for the different partons at several different momentum transfers and  known as PDFs\index{PDF} and are measured by DIS experiments.}
On the other hand, the initial transverse momentum is known to be zero\footnote{Apart from some intrinsic transverse momentum that the partons carry, which is negligible compared to the transverse momenta of the products of the scattering.}. So, in hadronic collision experiments, such as CDF, we are forced to use the missing transverse momentum (\vecpTmiss) as signature of elusive particles.

To determine~~\vecpTmiss\ we start with MET\index{MET}, which is defined as the negative vector sum of the transverse calorimetric energy\footnote{To avoid confusion, energy and momentum are treated equivalently, since the considered particles are highly relativistic.} of an event. 
%Particles, muons being the most characteristic example, do not necessarily deposit all of their energy in the calorimeter, either because they do not interact strongly and are \index{MIP}MIPs, or because they have enough energy for their showers to not be completely absorbed, or because some of their energy may escape through a crack of the detector.
As the energy deposited in the calorimeter is slightly offset with respect to the actual momentum of the produced objects, MET needs some readjustment for a more accurate determination of~~\vecpTmiss. 

The MET corrections involve adding the momentum of muons which is better known from their track curvature, as they are minimum ionizing particles and deposit a small fraction of their energy at the calorimeter. Also, the response of each calorimeter tower to electrons depends on the position in the tower where the electron enters it, and since that position is available from the electron track a correction to the response is taken into account, using calibration information from test beam. Finally, the measured jet energy is corrected for any non-linearity and energy loss in the un-instrumented regions of each calorimeter.
%level5-correction

After the reconstruction of final objects in an event, there typically is transverse energy that is not attributed to any object and is referred to as ``unclustered energy'' (\puncl). On the contrary, the ``clustered energy'' is defined as \Eclust, where the index $i$ runs through the reconstructed objects of the event. The three kinds of energy are related by
\begin{equation}
\Eclust + \vecpTmiss + \puncl = \vec{0},
\end{equation}
which can be used to determine \puncl\ with knowledge the other two quantities.

